Detecting Connectivity Issues in Android Apps

Android is the most popular mobile operating system in the world, running on more than 70% of mobile devices. This implies a gigantic and very competitive market for Android apps. Being successful in such a market is far from trivial and requires, besides the tackling of a problem or need felt by a vast audience, the development of high-quality apps. As recently showed in the literature, connectivity issues (e.g., mishandling of zero/unreliable Internet connection) can result in bugs and/or crashes, negatively affecting the app's user experience. While these issues have been studied in the literature, there are no techniques able to automatically detect and report them to developers. We present CONAN, a tool able to detect statically 16 types of connectivity issues affecting Android apps. We assessed the ability of CONAN to precisely identify these issues in a set of 44 open source apps, observing an average precision of 80%. Then, we studied the relevance of these issues for developers by (i) conducting interviews with six practitioners working with commercial Android apps, and (ii) submitting 84 issue reports for 27 open source apps. Our results show that several of the identified connectivity issues are considered as relevant by practitioners in specific contexts, in which connectivity is considered a first-class feature.

==> secs/content.tex <==
% !TEX root = ../main.tex

\section{Content}

Add all your missing sections here \\


\input{tables/dfltTable}

\begin{figure}[!h]
\centerline{\includegraphics[width=0.8\linewidth]{imgs/logoSquare.png}}
\caption{Example of a figure caption.}
\label{fig:test}
\end{figure}

All resources must be referenced using \lstinline[basicstyle=\small\ttfamily]|\fref{}|

\fref{lst:test}
\fref{fig:test}
\fref{tab:test}

\begin{lstlisting}[caption={test},label={lst:test}]
Test
\end{lstlisting}

In case the author needs to present a folder structure \textcolor{red}{dirtree} package can be used:

\begin{figure}[h]
	\centering
	\fbox{%
		\parbox{\dimexpr\linewidth-6\fboxsep-6\fboxrule}{%
			\fontsize{8pt}{8pt}
			\begin{minipage}[t]{\linewidth}
				\dirtree{%
					.1 /.
					.2 bin.
					.2 home.
					.3 jeancome.
					.4 texmf.
					.5 tex.
					.3 jeancomeson\DTcomment{Guillaume}.
					.3 jeancomedaughter\DTcomment{Mathilde}.
					.2 usr.
					.3 bin.
				}
			\end{minipage}\hfill
		}
	}
	\caption{Example Directory Tree}
	\label{fig:dirtree}
\end{figure}%



==> tables/dfltTable.tex <==
\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab:test}
\end{center}
\end{table}
